Model Collapse Demystified: The Case of Regression

In the era of proliferation of large language and image generation models, the phenomenon of "model collapse" refers to the situation whereby as a model is trained recursively on data generated from previous generations of itself over time, its performance degrades until the model eventually becomes completely useless, i.e the model collapses. In this work, we study this phenomenon in the setting of high-dimensional regression and obtain analytic formulae which quantitatively outline this phenomenon in a broad range of regimes. In the special case of polynomial decaying spectral and source conditions, we obtain modified scaling laws which exhibit new crossover phenomena from fast to slow rates. We also propose a simple strategy based on adaptive regularization to mitigate model collapse. Our theoretical results are validated with experiments.

==> related.tex <==
\section{Literature Overview}
\ElvisIssue{This section is too long (almost 2 pages...). It should be a single column worth of text (roughly).}

\ElvisIssue{This section was copied from "Big paper". We need to compress and adapt to the specific context of "Small paper".}

\paragraph{Model Collapse.} The phenomenon appeared in the {\em recent} literature in the context of language and image generation. Several recent works demonstrate facets of this phenomenon {\em empirically} in various settings \cite{Hataya_2023_ICCV, martínez2023combining,martínez2023understanding,bohacek2023nepotistically,briesch2023large,guo2023curious}. Only few recent works also provide some accompanying theoretical analysis \cite{shumailov2023curse,alemohammad2023selfconsuming,bertrand2023stability} which we outline now.

\cite{shumailov2023curse} define model collapse and attribute it to two mechanisms: finite sampling when training a model (leading to cut off of low-probability data) and function approximation errors (the model is not sufficiently expressive to model the true distribution). They observe (and, for a single Gaussian, prove) that upon iteratively resampling finite ''training data" the generated distribution becomes more and more peaked. Other models studied empirically are mixtures of (two) Gaussians and VAEs on MNIST. To study language models, \cite{shumailov2023curse} iteratively fine tune Meta's OPT-125M model on {\tt wikidata2}. For generation of new text they use a 5-way beam search, which, by its nature, (approximatively) generates only low-perplexity data. 

%\julia{I worry about the following statement from their paper \cite{shumailov2023curse}: {\em At the same time, we discover that generated data has much longer tails, suggesting that some of the data would never be produced by the original model – these are the errors that accumulate because of the learning with generational data.} If this is true, how can we possibly explain that? They also allude to the ''repeated text" problem of generated data, which is apparently already known.}
%\ElvisFix{Indeed, that sounds weird. I'll check their paper asap to see. Thanks for the info.}
% \ElvisIssue{Possible explanation is that: after many many generations, the generated data is straight up hallucination ? Unfortunately, we can't probe / reproduce this phenomenon using our (currently) toy LLM discrete setup (the support of the data only reduces after each generation).} \julia{What if we add some noise to the model output? But why would that generate extra tail? Truly weird. But they are very (VERY) sloppy in their paper, so maybe this just isn't reproducible. They do not observe this in the GM or VAE setting, just in their weird LLM setup.}

\julia{I commented out our chatter here, but let's keep a note on the purportedly longer tails from AI-generation (because who knows, we might be able to prove something theoretically) and mention the repeated-text problem of regenerated data.}

 \cite{alemohammad2023selfconsuming}  conduct an empirical and analytical analysis on generative image models of what they term the ''self-consuming" or ''autophaguous" loop. They conclude that without enough fresh real data at each generation, future models necessarily will have their precision or recall decrease. They model the influence of each new AI-generation via a generic {\em sampling bias} $0 \leq \lambda \leq 1 $. In the case of image generation this refers to feature parameters at generation that favor quality over diversity (suitably quantified). More precisely, $\lambda=1$ corresponds to unbiased sampling and $\lambda=0$ corresponds to sampling from the modes of the generative distribution. $\lambda$  models biased sampling methods commonly used in generative modeling practice, such as truncation in BigGAN and StyleGAN or guidance in diffusion models. 
 In the case of Gaussian distributions, $\lambda$ is the shrinking factor of the variance of the next generation. Their empirical work studies GANs and denoising diffusion probabilistic models for image generation on FFHQ and MNIST and single Gaussians for both theoretical and empirical observations. As in \cite{shumailov2023curse} they observe (and prove for the case of a single Gaussian) that estimation error alone leads to vanishing variance with number of iterations.
 \cite{alemohammad2023selfconsuming} also empirically observe an initial boost in performance in a regime where modest amounts of synthetic data are mixed with the original data before larger amounts of synthetic data lead to ultimate degradation. This might mimick larger-scale results that demonstrate how synthetic data mixed with true data improves performance in some scenarios (see {\em Benefits of synthesized data} below).  \julia{Ok, Elvis, I am really counting on you getting an analytical mixing phase transition here!} Indeed, in its simplest form, data augmentation (rotations, cropping etc.~), a widespread highly beneficial practice in ML training, can be viewed as the simplest form of data generation.


A concurrent paper \cite{bertrand2023stability} on image generation \julia{Continue here.} {\em we develops a framework to rigorously study the impact of training generative models on mixed datasets (of real and synthetic data) on their stability. We first prove the stability of iterative training under the condition that the initial generative models approximate the data distribution well enough and the proportion of clean training data (w.r.t. synthetic data) is large enough. We empirically validate our theory on both synthetic and natural images by iteratively training normalizing flows and state-of-the-art diffusion models on CIFAR10 and FFHQ.} \julia{read, check and summarize.}

Several empirical studies confirm the deleterious effect of training on self-generated data: In the context of image generation, 
\cite{martínez2023combining,martínez2023understanding} report  degradation of models trained on AI-generated data. Specifically, they use a Denoising Diffusion Implicit Model and a few (relatively small) datasets (e.g.~Orchids, MNIST) to demonstrate visual degradation when training in successive generations of AI-generated data. 
\cite{Hataya_2023_ICCV} {\em ''conclude that generated images negatively affect downstream performance, while the significance depends on tasks and the amount of generated images"}, \cite{bohacek2023nepotistically} reports that the popular StableDiffusion model collapses when iteratively retrained on self-generated faces, even with as little as $3\%$ synthetic data mixed into the original training set. For text, \cite{briesch2023large} use {\em nanoGPT}\footnote{\tt https://github.com/karpathy/nanoGPT} on a curated 10K logical-expression dataset to demonstrate the iterative collapse of self-consuming loops - the model and dataset are sufficiently small to allow training from scratch. \cite{guo2023curious} observe a decline in linguistic diversity metrics across iteratively fine-tuned LLMs. \julia{Continue}


\paragraph{Scaling Laws.}
Neural scaling laws have been observed empirically in vision, language and speech. 
% \ElvisIssue{Also mention the case regression (the focus of this paper), and discuss \cite{Caponnetto2007OptimalRF,Spigler_2020,Cui_2022}, etc.}
An early large scale empirical study is performed in \cite{hestness2017deep}, demonstrating power law scaling across a range of learning scenarios. This is followed by  well-known studies from OpenAI
\cite{kaplan2020scaling} and DeepMind \cite{hoffmann2022trainingChinchilla}, which empirically demonstrate power-law scaling in LLMs across a wide set of scales. Essentially, this empirically establishes that 
$$L(T,P) \approx L_0 + C_1 T^{-c_1} + C_2 P^{-c_2},$$ where $L$ is the per-token cross entropy loss (in nats), $T,P$ are the number of (non-embedding) parameters and data, respectively, and $C_1, C_2$ and $c_1,c_1$ are constants determined by the data distribution and the model specifications. 



This study was extended in a follow up \cite{henighan2021scaling}  to demonstrate many more power law relations in various scenarios (vision transformer, video modeling, multimodal models, and mathematical problem solving. In \cite{gordon-etal-2021-data}, for the machine translation (MT) setting, scaling laws for standard benchmarks like BLEU are quantified and explained via cross-entropy power-law scaling, thus positing a first universality of scaling laws across metrics. \cite{hernandez2021scaling} demonstrate similar empirical power-law scaling for transfer learning. 

\paragraph{Theoretical Models for Scaling Laws.} 
\julia{I need to check out \cite{rosenfeld2019constructive}. Then list Maloney, Hutter, EVA. There is also the Tegmark ``Quantization" paper \cite{michaud2023the}. }

From a theoretical angle, scaling laws have been shown analytically even before the emergence of large foundation models. For instance, \cite{Caponnetto2007OptimalRF} characterize the power-law generalization error of regularized least-squares kernel algorithms.
More recently, scaling laws have been shown for kernel models under the Gaussian design, e.g. in \cite{Cui_2022}. To our knowledge, however, very few papers deal with the decay of scaling in the case of self-consuming loops. A notable example is \cite{bartlett2020neurips} which studies \julia{to be continued}

